Extending Data Spatial Semantics for Scale Agnostic Programming

We introduce extensions to Data Spatial Programming (DSP) that enable scale-agnostic programming for application development. Building on DSP's paradigm shift from data-to-compute to compute-to-data, we formalize additional intrinsic language constructs that abstract persistent state, multi-user contexts, multiple entry points, and cross-machine distribution for applications. By introducing a globally accessible root node and treating walkers as potential entry points, we demonstrate how programs can be written once and executed across scales, from single-user to multi-user, from local to distributed, without modification. These extensions allow developers to focus on domain logic while delegating runtime concerns of persistence, multi-user support, distribution, and API interfacing to the execution environment. Our approach makes scale-agnostic programming a natural extension of the topological semantics of DSP, allowing applications to seamlessly transition from single-user to multi-user scenarios, from ephemeral to persistent execution contexts, and from local to distributed execution environments.

==> listings.tex <==
%----------------------------------- LISTINGS  ------------------------------
% define a new language definition for YAML
\lstdefinelanguage{yaml}{
  keywords={true,false,null,y,n},
  keywordstyle=\color{darkgray}\bfseries,
  sensitive=false,
  comment=[l]{\#},
  commentstyle=\color{purple}\ttfamily,
  stringstyle=\color{blue}\ttfamily,
  morestring=[b]',
  morestring=[b]"
}

% % Basic styling for listings
% \lstdefinelanguage{python}{
%     % list of keywords
%    keywords={ import, node, ignore, take, entry, activity, exit, spawn, 
%            edge, walker, or, if, elif, else, for,  by, while,
%            continue, break, disengage, report, anchor, has, can, true, false, from,
%            context, info, details, try, strict, length, test, type, str,
%            int, float, list, dict, bool, digraph, subgraph, test, by, 
%            skip, assert, yield, class, def, Method, Function, pass,except,strip,split,obj,glob
%        },
%    sensitive=false, % keywords are not case-sensitive
%    morecomment=[l]{//}, % l is for line comment
%    morecomment=[l]{\#}, % l is for line comment
%    morecomment=[s]{/}{/}, % s is for start and end delimiter
%    morecomment=[s]{```}{```}, % s is for start and end delimiter
%    % moredelim=[s][\color{orange}]{f"}{"}, % Color f-strings with double quotes
%    % moredelim=[s][\color{orange}]{f'}{'}, % Color f-strings with single quotes
%    % moredelim=[is][\color{blue}]{\{}{\}}, % Color code 
%    % stringstyle=\color{orange},
%    morestring=[b]", % defines that strings are enclosed in double quotes
%    morestring=[b]',
%    % morestring=[b]`,
%    morestring=[s][]{\{}{\}}
%    % morestring=[b]f", % Add support for f-strings
%    % morestring=[b]f',
% }

% \lstset{
%   language = yaml,
%   basicstyle=\fontsize{8}{10}\upshape\ttfamily,
%   columns=fullflexible,
%   breaklines=true,
%   captionpos=b,
%   showstringspaces=false, % Do not show spaces as special characters
%   frame=single, % Adds a frame around the code
%   xleftmargin=10pt, %5.8
%   xrightmargin=10pt,
%   %postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space}, % For indicating wrapped lines
% }

% % Python style for highlighting
% \newcommand\pythonstyle{\lstset{
%     language=Python,
%     frame=single,                                    % adds a frame around the code
%     columns=fullflexible,
%     breaklines=true,
%     % postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space},
%     % backgroundcolor=\color{gray!10},
%     captionpos=t,
%     basicstyle=\fontsize{6pt}{5pt}\upshape\ttfamily,      % the size of the fonts that are used for the code
%     numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
%     numbersep=8pt,                   % how far the line-numbers are from the code
%     numberstyle=\tiny\color{gray}, % the style that is used for the line-numbers
%     keywordstyle=\bfseries\color{blue!55!black},
%     %    commentstyle=\itshape\color{purple!70!black},
%     %    identifierstyle=\color{blue!80!black},
%     stringstyle=\color{orange},
%     xleftmargin=5pt, %5.8
%     xrightmargin=10pt,
%     commentstyle=\color{gray}\ttfamily,
%     backgroundcolor=\color{white},
%     morekeywords={self},              % Add keywords here
%     % keywordstyle=\ttb\color{deepblue},
%     emph={MyClass,__init__,return,type, str, int,
%                int, float, list, dict, bool,tuple},          % Custom highlighting
%     emphstyle=\bfseries\color{green!50!black},    % Custom highlighting style
%     frame=tb,                         % Any extra options here
%     showstringspaces=false
% }

% }


% % Python environment
% \lstnewenvironment{python}[1][]
% {
% \pythonstyle
% \lstset{#1}
% }
% {}

% % Python for inline
% \newcommand\pythoninline[1]{{\pythonstyle\lstinline!#1!}}

% Custom colors for additions and deletions in diff-style code
\definecolor{addition}{rgb}{0, 0.6, 0} % Green for additions
\definecolor{deletion}{rgb}{0.8, 0, 0} % Red for deletions
\definecolor{unchanged}{rgb}{0, 0, 0}  % Black for unchanged code

% % Diff environment
% \lstnewenvironment{pythondiff}[1][]
% {
%     \pythonstyle
%     \lstset{
%         showspaces=false,                          % Don't show spaces explicitly
%         showtabs=false,                            % Don't show tabs explicitly
%         columns=fixed,                             % Ensure fixed-width columns to preserve indentation
%         keepspaces=true,                           % Preserve spaces and indentation
%         % language for highlighting changes
%         morecomment=[f][\color{deletion}]{-},       % Red for deletions
%         morecomment=[f][\color{addition}]{+},       % Green for additions
%         morecomment=[f][\color{unchanged}]{ },      % Black for unchanged lines
%         moredelim=[il][\color{deletion}\sout]{\-},  % Strikethrough for deleted lines
%         moredelim=[il][\color{addition}]{\+},       % Color added lines green
%         % frame=single,                               % Keep the frame styling
%         % columns=fullflexible,                       % Keep flexible column width
%         % breaklines=true,                            % Line breaks
%         % backgroundcolor=\color{gray!10},            % Light gray background
%         % captionpos=t,
%         % basicstyle=\fontsize{6}{5}\upshape\ttfamily, % Keep your basic style
%         % numbers=left,
%         % numbersep=8pt,
%         % numberstyle=\tiny\color{gray},
%         % keywordstyle=\bfseries\color{blue!55!black},
%         % stringstyle=\color{orange},
%         % xleftmargin=5pt,
%         % xrightmargin=10pt,
%         % commentstyle=\color{gray}\ttfamily,
%         % showstringspaces=false,
%         % emphstyle=\bfseries\color{green!50!black},  % Custom highlighting style
%         % morekeywords={self,model,llm},
%         literate=                                  % Preserve indentation and highlight diffs
%         {-}{{\color{deletion}-}}1                  % Red for deletions
%         {+}{{\color{addition}+}}1                  % Green for additions
%         {^}{{\ }}1 
%         #1 % Additional user-defined options
%     }
% }
% {}

\lstdefinelanguage{jac}{
        % list of keywords
       keywords={ import, node, ignore, take, activity, exit, spawn,
               edge, walker, and, or, if, elif, else, for, with, by, while, for, return,report, 
               continue, break, disengage, report, anchor, has, can, true, false, from, root, 
               context, info, details, try, strict, length, test, digraph, subgraph, test, by, in, to,
               skip, assert, yield, class, obj, Method, can, glob, from
           },
       sensitive=false, % keywords are not case-sensitive
       commentstyle=\color{purple}\ttfamily,
       morecomment=[l]{//}, % l is for line comment
       morecomment=[l]{\#}, % l is for line comment
       % morecomment=[s]{/}{/}, % s is for start and end delimiter
       % morecomment=[s]{```}{```}, % s is for start and end delimiter
       morestring=[b]", % defines that strings are enclosed in double quotes
       morestring=[b]',
       % morestring=[b]`,
       % morestring=[s][]{\{}{\}}
    }
    
    \lstset{
        language=jac,
        % aboveskip=0pt,
        % belowskip=0pt,
        frame=single,
        columns=fullflexible,
        breaklines=true,
        % backgroundcolor=\color{gray!10},
        captionpos=t,
        basicstyle=\fontsize{6}{5}\upshape\ttfamily,
        numbers=left,
        numbersep=8pt,
        numberstyle=\tiny\color{gray},
        keywordstyle=\bfseries\color{blue!55!black},
        stringstyle=\color{orange},
        xleftmargin=5pt,
        xrightmargin=10pt,
        backgroundcolor=\color{white},
        morekeywords={self},
        % keywordstyle=\ttb\color{deepblue},
        emph={return,by,py,jac,entry,type, str, int, root,
               int, float, list, dict, bool},
        emphstyle=\bfseries\color{green!50!black},
        frame=tb,                         % Any extra options here
        showstringspaces=false
    }

% % Jaclang style for highlighting
% \newcommand\jacstyle{
%     \lstdefinelanguage{jac}{
%         % list of keywords
%        keywords={ import, node, ignore, take, activity, exit, spawn, with,
%                edge, walker, and, or, if, elif, else, for, with, by, while,
%                continue, break, disengage, report, anchor, has, can, true, false, from,
%                context, info, details, try, strict, length, test, digraph, subgraph, test, by, in, to,
%                skip, assert, yield, class, obj, Method, can, glob, from
%            },
%        sensitive=false, % keywords are not case-sensitive
%        morecomment=[l]{//}, % l is for line comment
%        morecomment=[l]{\#}, % l is for line comment
%        morecomment=[s]{/}{/}, % s is for start and end delimiter
%        % morecomment=[s]{```}{```}, % s is for start and end delimiter
%        morestring=[b]", % defines that strings are enclosed in double quotes
%        morestring=[b]',
%        % morestring=[b]`,
%        morestring=[s][]{\{}{\}}
%     }
    
%     \lstset{
%         language=jac,
%         % aboveskip=0pt,
%         % belowskip=0pt,
%         frame=single,
%         columns=fullflexible,
%         breaklines=true,
%         % backgroundcolor=\color{gray!10},
%         captionpos=t,
%         basicstyle=\fontsize{6}{5}\upshape\ttfamily,
%         numbers=left,
%         numbersep=8pt,
%         numberstyle=\tiny\color{gray},
%         keywordstyle=\bfseries\color{blue!55!black},
%         stringstyle=\color{orange},
%         xleftmargin=5pt,
%         xrightmargin=10pt,
%         backgroundcolor=\color{white},
%         morekeywords={self},
%         % keywordstyle=\ttb\color{deepblue},
%         emph={return,by,py,jac,entry,type, str, int,
%                int, float, list, dict, bool},
%         emphstyle=\bfseries\color{green!50!black},
%         frame=tb,                         % Any extra options here
%         showstringspaces=false
%     }

% }

% % % jaclang for inline
% \newcommand\jacinline[1]{{\jacstyle\lstinline!#1!}}

% % JAC style environment
% \lstnewenvironment{jac}[1][]
%     {
%     \leavevmode
%     \jacstyle
%     \lstset{#1}
%     }
% {}

% Command to input listing from jac file
% \newcommand{\jacinputlisting}[2][]{%
%     \jacstyle%
%     \lstinputlisting[#1]{#2}%
% }


% \lstdefinelanguage{output}{
%     keywords={Output},
%     basicstyle=\tiny\ttfamily, 
%     breaklines=true,
%     keywordstyle=\color{blue},
%     stringstyle=\color{black},
%     commentstyle=\color{gray},
%     morecomment=[l]{//},
%     columns=fullflexible,
%     xleftmargin=15pt,
%     xrightmargin=5pt,
%     showstringspaces=false
% }

% \lstdefinelanguage{vision_output}{
%     keywords={Output},
%     basicstyle=\tiny\ttfamily, 
%     breaklines=true,
%     keywordstyle=\color{blue},
%     stringstyle=\color{black},
%     commentstyle=\color{gray},
%     morecomment=[l]{//},
%     columns=fullflexible,
%     xleftmargin=5pt,
%     xrightmargin=5pt,
%     showstringspaces=false
% }

\newcommand{\pyinputlisting}[2][]{%
    \lstinputlisting[#1]{#2}%
}
